GaIA: Graphical Information Gain based Attention Network for Weakly Supervised Point Cloud Semantic Segmentation

While point cloud semantic segmentation is a significant task in 3D scene understanding, this task demands a time-consuming process of fully annotating labels. To address this problem, recent studies adopt a weakly supervised learning approach under the sparse annotation. Different from the existing studies, this study aims to reduce the epistemic uncertainty measured by the entropy for a precise semantic segmentation. We propose the graphical information gain based attention network called GaIA, which alleviates the entropy of each point based on the reliable information. The graphical information gain discriminates the reliable point by employing relative entropy between target point and its neighborhoods. We further introduce anchor-based additive angular margin loss, ArcPoint. The ArcPoint optimizes the unlabeled points containing high entropy towards semantically similar classes of the labeled points on hypersphere space. Experimental results on S3DIS and ScanNet-v2 datasets demonstrate our framework outperforms the existing weakly supervised methods. We have released GaIA at https://github.com/Karel911/GaIA.

==> table/ablation_loss.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of mIoU with respect to three loss functions on ScanNet-v2 validation set. ($\cdot$) indicates officially measured test scores.}
\resizebox{0.4\textwidth}{!}{%
{\Large
\label{table_ablation_loss}
\begin{tabular}{ccc|cc}
\hline
Sia. & ArcFace & ArcPoint & 1pt & 1\%\\
\hline
\checkmark & & & 40.8 & 52.4\\
\checkmark & \checkmark & & 41.1 & 52.8\\
\multirow{2}{*}{\checkmark} &  & \multirow{2}{*}{\checkmark} & 41.9 & 54.9\\
& & & ({\bf 52.1}) & ({\bf 65.3})\\
\hline
\end{tabular}}}
\end{table}

==> table/area5.tex <==
% \newcommand{\etal}{\textit{et al.}}

\begin{table*}[ht]
\centering
\caption{Comparison with existing methods and baselines on S3DIS area 5.}
\resizebox{1.0\textwidth}{!}{%
{\Large
\label{area5}
\begin{tabular}{c|c|c|cccccccccccccc}
\hline
Method & Sup. & mIoU & ceil. & floor & wall & beam & col. & win. & door & chair & table & book. & sofa & board & clu.\\

\hline

PointNet \cite{qi2017pointnet}    & 100\% & 41.1 & 88.8 & 97.3 & 69.8 & 0.1 & 3.9 & 46.3 & 10.8 & 59.0 & 52.6 & 5.9 & 40.3 & 26.4 & 33.2 \\ % Point Transformer(ICCV 2021)
SegCloud \cite{Tchapmi2017SEGCloudSS} & 100\% & 48.9 & 90.1 & 96.1 & 69.9 & 0.0 & 18.4 & 38.4 & 23.1 & 70.4 & 75.9 & 40.9 & 58.4 & 13.0 & 41.6  \\ % Point Transformer(ICCV 2021)
PointCNN \cite{Li2018PointCNNCO}      & 100\% & 57.3 & 92.3 & 98.2 & 79.4 & 0.0 & 17.6 & 22.8 & 62.1 & 74.4 & 80.6 & 31.7 & 66.7 & 62.1 & 56.7\\ % Point Transformer(ICCV 2021)
RandLA-Net \cite{hu2020randla} & 100\% & 63.0 & 92.4 & 96.7 & 80.6 & 0.0 & 18.3 & 61.3 & 43.3 & 77.2 & 85.2 & 71.5 & 71.0 & 69.2 & 52.3 \\ % PSD(CVPR 2021)
PSD \cite{zhang2021perturbed} & 100\% & 65.1 & 92.3 & 97.1 & 80.7 & 0.0 & 32.4 & 55.5 & 68.1 & 78.9 & 86.8 & 71.1 & 70.6 & 59.0 & 53.0\\ % PSD(CVPR 2021)
MinkowskiNet \cite{choy20194d} & 100\% & 65.4 & 91.8 & 98.7 & 86.2 & 0.0 & 34.1 & 48.9 & 62.4 & 89.8 & 81.6 & 74.9 & 47.2 & 74.4 & 58.6 \\ % MinkowskiNet (CVPR 2019)
KPConv \cite{thomas2019KPConv} & 100\% & 67.1 & 92.8 & 97.3 & 82.4 & 0.0 & 23.9 & 58.0 & 69.0 & 81.5 & 91.0 & 75.4 & 75.3 & 66.7 & 58.9\\ % Point Transformer(ICCV 2021)
PointTransformer \cite{zhao2021point} &100\% & 70.4 & 94.0 & 98.5 & 86.3 & 0.0 & 38.0 & 63.4 & 74.3 & 89.1 & 82.4 & 74.3 & 80.2 & 76.0 & 59.3 \\ % Point Transformer(ICCV 2021)
VoteNet \cite{hou2021exploring} & 100\% & \bf 72.2 & 95.1 & 98.4 & 86.3 & 0.0 & 40.7 & 60.8 & 85.2 & 91.8 & 81.9 & 73.9 & 78.9 & 82.8 & 62.4 \\ % CVPR 2021
Baseline (Ours) & 100\% & 60.3 & 92.4 & 92.5 & 78.5 & 0.4 & 22.3 & 71.9 & 75.8 & 65.1 & 57.9 & 38.2 & 42.7 & 48.7 & 52.2 \\
\hline

% Xu and Lee \cite{xu2020weakly} & 10\% & 48.0 & 90.1 & 97.1 & 71.9 & 0.0 & 1.9 & 47.2 & 29.3 & 62.9 & 64.0 & 15.9 & 42.2 & 18.9 & 37.5\\ % PSD(CVPR 2021)
% \hline

Zhang \etal \cite{zhang2021weakly} & 1\% & 61.8 & 91.5 & 96.9 & 80.6 & 0.0 & 18.2 & 58.1 & 47.2 & 75.8 & 85.7 & 65.2 & 68.9 & 65.0 & 50.2\\ % PSD(CVPR 2021)
PSD \cite{zhang2021perturbed} & 1\% & 63.5 & 92.3 & 97.7 & 80.7 & 0.0 & 27.8 & 56.2 & 62.5 & 78.7 & 84.1 & 63.1 & 70.4 & 58.9 & 53.2 \\ % PSD(CVPR 2021)
Baseline (Ours) & 1\% & 57.8 & 91.5 & 92.2 & 75.3 & 0.6 & 20.2 & 67.4 & 68.8 & 62.3 & 50.8 & 33.8 & 33.4 & 46.5 & 44.8\\
GaIA (Ours) & 1\% & \bf 69.1 & 93.7 & 98.2 & 84.2 & 1.8 & 33.2 & 60.5 & 72.6 & 86.7 & 86.4 & 70.2 & 77.6 & 73.2 & 59.7\\
\hline

Xu and Lee \cite{xu2020weakly} & 1pt & 44.5 & 90.9 & 97.3 & 74.8 & 0.0 & 8.4 & 49.3 & 27.3 & 69.0 & 71.7 & 16.5 & 53.2 & 23.3 & 42.8\\ % PSD(CVPR 2021)
PSD \cite{zhang2021perturbed} & 1pt & 48.2 & 87.9 & 96.0 & 62.1 & 0.0 & 20.6 & 49.3 & 40.9 & 55.1 & 61.9 & 43.9 & 50.7 & 27.3 & 31.1 \\% PSD(CVPR 2021)
GaIA (Ours) & 1pt & 63.2 & 93.2 & 94.6 & 76.0 & \textbf{69.2} & 31.9 & 74.8 & 72.6 & 64.8 & 57.4 & 40.1 & 42.9 & 49.4 & 54.2\\ 

\hline
\end{tabular}}}
\end{table*}


